The multiplicity distribution of Kepler's exoplanets

The true multiplicity distribution of transiting planet systems is obscured by strong observational biases, leading low-multiplicity systems to be overrepresented in the observed sample. Using the Kepler FGK planet hosts, we employ approximate Bayesian computation to infer the multiplicity distribution by comparing simulated catalogs to the observed one. After comparing a total of ten different multiplicity distributions, half of which were two-population models, to the observed data, we find that a single-population model following a Zipfian distribution is able to explain the Kepler data as well as any of the dichotomous models we test. Our work provides another example of a way to explain the observed Kepler multiplicities without invoking a dichotomous planet population. Using our preferred Zipfian model, we estimate that an additional $2393_{-717}^{+904}$ planets likely reside in the 1537 FGK Kepler systems studied in this work, which would increase the planet count by a factor of $2.22_{-0.36}^{+0.46}$. Of these hidden worlds, $663_{-151}^{+158}$ are expected to reside in ostensibly single-transiting-planet systems, meaning that an additional planet(s) is expected for approximately 1-in-2 such Kepler systems.

==> fakesAICtable.tex <==
\begin{table}
\caption{The Akaike information criterion calculated for four model fits to simulated multiplicity distributions. The ``true model" refers to the model used to generate the multiplicity distribution, and the ``tested model" refers to the model used to fit it.} % title of Table
\centering % used for centering table
\begin{tabular}{c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Tested model & True model & AIC\\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
Poisson & Poisson & $37.954\pm2.872$\\
Zipf & Poisson & $38.367\pm2.872$\\
Poisson & Zipf & $53.602\pm2.872$\\
Zipf & Zipf & $40.488\pm2.872$\\ [1ex]
\hline\hline %inserts single line
\end{tabular}
\label{tab:fakeAICs} % is used to refer this table in the text
\end{table}

==> post_fakes.tex <==
\begin{table*}
\caption{\emph{Comparison of the a-posteriori parameters from fitting the fake data
sets to the true injected values. We list the median and 1\,$\sigma$ credible interval
for each parameter.}} % title of Table
\centering % used for centering table
\begin{tabular}{c c c c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Experiment & $\alpha_{\mathrm{small}}$ & $\alpha_{\mathrm{big}}$ & $R_{\mathrm{crit}}$\,[$R_{\oplus}$] & $\alpha$ & $\sigma_I$\,[$^{\circ}$] \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
Poisson Model \\
\hline
Truth & 0.33 & 5.00 & 2.50 & 5.00 & 2.00 \\
1	& $0.13_{-0.23}^{+0.39}$ & $4.82_{-0.73}^{+0.85}$ & $2.54_{-0.31}^{+0.30}$ & $5.06_{-0.93}^{+0.91}$ & $1.72_{-0.54}^{+0.52}$ \\
2	& $0.10_{-0.25}^{+0.31}$ & $6.01_{-1.34}^{+2.01}$ & $2.86_{-0.37}^{+0.39}$ & $4.98_{-0.99}^{+1.36}$ & $1.66_{-0.64}^{+0.48}$ \\
3	& $0.00_{-0.20}^{+0.32}$ & $5.49_{-1.01}^{+1.81}$ & $2.86_{-0.40}^{+0.40}$ & $5.18_{-1.09}^{+1.05}$ & $1.80_{-0.50}^{+0.57}$ \\
4	& $0.12_{-0.22}^{+0.29}$ & $5.46_{-1.01}^{+1.76}$ & $2.74_{-0.36}^{+0.41}$ & $4.90_{-1.05}^{+1.63}$ & $1.61_{-0.45}^{+0.40}$ \\
5	& $0.17_{-0.22}^{+0.25}$ & $5.60_{-0.98}^{+1.54}$ & $2.74_{-0.30}^{+0.33}$ & $5.54_{-1.20}^{+0.92}$ & $1.27_{-0.51}^{+0.36}$ \\
6	& $0.23_{-0.28}^{+0.29}$ & $5.34_{-0.81}^{+1.23}$ & $2.65_{-0.27}^{+0.39}$ & $5.15_{-1.05}^{+1.77}$ & $1.68_{-0.52}^{+0.44}$ \\
7	& $0.15_{-0.21}^{+0.30}$ & $5.66_{-1.00}^{+1.68}$ & $2.77_{-0.28}^{+0.37}$ & $5.05_{-0.96}^{+1.29}$ & $1.43_{-0.49}^{+0.41}$ \\
8	& $0.11_{-0.22}^{+0.26}$ & $5.68_{-0.97}^{+1.51}$ & $2.74_{-0.25}^{+0.39}$ & $4.99_{-1.46}^{+1.77}$ & $1.70_{-0.55}^{+0.43}$ \\
9	& $0.15_{-0.23}^{+0.23}$ & $5.07_{-0.77}^{+1.21}$ & $2.63_{-0.26}^{+0.33}$ & $4.65_{-0.79}^{+0.89}$ & $1.63_{-0.48}^{+0.40}$ \\
10	& $0.37_{-0.33}^{+0.27}$ & $5.18_{-0.71}^{+0.87}$ & $2.57_{-0.20}^{+0.26}$ & $5.00_{-1.82}^{+1.76}$ & $2.02_{-0.49}^{+0.36}$ \\
\hline
Zipfian Model \\
\hline
Truth & 0.33 & 5.00 & 2.50 & 1.00 & 2.00 \\
1	& $0.52_{-0.28}^{+0.38}$ & $4.77_{-0.68}^{+0.89}$ & $2.44_{-0.25}^{+0.25}$ & $0.70_{-0.27}^{+0.26}$ & $3.24_{-1.01}^{+1.22}$ \\
2	& $0.32_{-0.23}^{+0.33}$ & $4.90_{-0.68}^{+1.31}$ & $2.42_{-0.26}^{+0.35}$ & $0.97_{-0.17}^{+0.13}$ & $1.79_{-0.53}^{+0.76}$ \\
3	& $0.26_{-0.23}^{+0.36}$ & $4.97_{-0.74}^{+1.65}$ & $2.62_{-0.33}^{+0.38}$ & $0.95_{-0.18}^{+0.16}$ & $2.54_{-0.77}^{+0.90}$ \\
4	& $0.38_{-0.28}^{+0.32}$ & $5.24_{-0.80}^{+0.91}$ & $2.52_{-0.26}^{+0.26}$ & $0.83_{-0.24}^{+0.21}$ & $2.67_{-0.89}^{+1.29}$ \\
5	& $0.20_{-0.22}^{+0.27}$ & $4.98_{-0.65}^{+1.11}$ & $2.57_{-0.25}^{+0.30}$ & $0.81_{-0.24}^{+0.17}$ & $2.12_{-0.74}^{+0.94}$ \\
6	& $0.36_{-0.24}^{+0.32}$ & $4.82_{-0.64}^{+0.81}$ & $2.54_{-0.22}^{+0.27}$ & $0.48_{-0.39}^{+0.32}$ & $3.88_{-1.03}^{+1.53}$ \\
7	& $0.44_{-0.27}^{+0.39}$ & $5.07_{-0.58}^{+0.89}$ & $2.47_{-0.22}^{+0.27}$ & $1.07_{-0.16}^{+0.12}$ & $1.99_{-0.64}^{+0.76}$ \\
8	& $0.23_{-0.21}^{+0.25}$ & $5.32_{-0.77}^{+1.13}$ & $2.68_{-0.23}^{+0.28}$ & $0.83_{-0.20}^{+0.17}$ & $2.41_{-0.74}^{+0.86}$ \\
9	& $0.26_{-0.23}^{+0.33}$ & $5.15_{-0.78}^{+1.63}$ & $2.61_{-0.30}^{+0.35}$ & $1.10_{-0.19}^{+0.14}$ & $1.63_{-0.64}^{+0.75}$ \\
10	& $0.61_{-0.34}^{+0.44}$ & $4.76_{-0.65}^{+0.95}$ & $2.39_{-0.29}^{+0.34}$ & $0.71_{-0.26}^{+0.24}$ & $3.62_{-1.19}^{+1.13}$ \\ [1ex]
\hline\hline %inserts single line
\end{tabular}
\label{tab:postfakes} % is used to refer this table in the text
\end{table*}
